A Comparison of the Effects of Neutron and Gamma Radiation in Silicon Photomultipliers

The effects of radiation damage in silicon photomultipliers (SiPMs) from gamma rays have been measured and compared with the damage produced by neutrons. Several types of MPPCs from Hamamatsu were exposed to gamma rays and neutrons at the Solid State Gamma Ray Irradiation Facility (SSGRIF) at Brookhaven National Lab and the Institute for Nuclear Research (Atomki) in Debrecen, Hungary. The gamma ray exposures ranged from 1 krad to 1 Mrad and the neutron exposures ranged from 10$^8$ n/cm$^2$ to 10$^{12}$ n/cm$^2$. The main effect of gamma ray damage is an increase in the noise and leakage current in the irradiated devices, similar to what is seen from neutron damage, but the level of damage is considerably less at comparable high levels of exposure. In addition, the damage from gamma rays saturates after a few hundred krad, while the damage from neutrons shows no sign of saturation, suggestive of different damage mechanisms in the two cases. The change in optical absorption in the window material of the SiPMs due to radiation was also measured. This study was carried out in order to evaluate the use of SiPMs for particle physics applications with moderate levels of radiation exposures.

==> conclusions.tex <==
\label{sec:conclusions}



==> results.tex <==
\label{sec:results}
\label{results}

\begin{figure}[!hbt]
  \begin{center}
%   \includegraphics[width=\linewidth,trim={2cm 0 5cm 0},clip]{figs/getMeanRMS_Summary_rootFitVerticalScan.pdf}
 \end{center}
%  \caption{EMCal MIP peak amplitude plotted against the beam position along the length of module. The data points, %which are the average response from eight towers, are fit with an exponential function (curve).}
%  \label{fig:attenuation}
\end{figure}


